3-D selection of 167 sub-stellar companions to nearby stars

We analyze 5108 AFGKM stars with at least five high precision radial velocity points as well as Gaia and Hipparcos astrometric data utilizing a novel pipeline developed in previous work. We find 914 radial velocity signals with periods longer than 1000\,d. Around these signals, 167 cold giants and 68 other types of companions are identified by combined analyses of radial velocity, astrometry, and imaging data. Without correcting for detection bias, we estimate the minimum occurrence rate of the wide-orbit brown dwarfs to be 1.3\%, and find a significant brown dwarf valley around 40 $M_{\rm Jup}$. We also find a power-law distribution in the host binary fraction beyond 3 au similar to that found for single stars, indicating no preference of multiplicity for brown dwarfs. Our work also reveals nine sub-stellar systems (GJ 234 B, GJ 494 B, HD 13724 b, HD 182488 b, HD 39060 b and c, HD 4113 C, HD 42581 d, HD 7449 B, and HD 984 b) that have previously been directly imaged, and many others that are observable at existing facilities. Depending on their ages we estimate that an additional 10-57 sub-stellar objects within our sample can be detected with current imaging facilities, extending the imaged cold (or old) giants by an order of magnitude.

==> fitting_plot.tex <==
\begin{figure}
\includegraphics[scale=0.6]{{{GJ234_N0_fit}}}
\includegraphics[scale=0.6]{{{GJ3222_N0_fit}}}
\includegraphics[scale=0.6]{{{GJ3677_N0_fit}}}
\includegraphics[scale=0.6]{{{GJ3962_N0_fit}}}
\includegraphics[scale=0.6]{{{GJ570A_N0_fit}}}
\caption{Combined RV and astrometry fit for all brown dwarf targets. The left panels show the RV fits,
    the middle ones show proper motion fit, and the right ones show
    position fit. For each target, the linear motion is subtracted from the
    proper motion and position to show planet-induced nonlinear
    motion. The RV data sets as well as Gaia and Hipparcos astrometric
    data are encoded by the same colors as shown by the left-hand legends. The
    covariances of the Gaia and Hipparcos proper motions and positions
    are denoted by error ellipses. The straight line connects the data point
    to the best fitting model, which represents where the companion is
    expected to be. The parameters at the MAP are shown on the right side of the figure. }
\label{fig:fit1}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{GJ660.1_N0_fit}}}
\includegraphics[scale=0.6]{{{GJ680_N0_fit}}}
\includegraphics[scale=0.6]{{{GJ864_N0_fit}}}
\includegraphics[scale=0.6]{{{GJ9714_N0_fit}}}
\includegraphics[scale=0.6]{{{HD101065_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD105618_N0_fit}}}
\includegraphics[scale=0.6]{{{HD109988_N0_fit}}}
\includegraphics[scale=0.6]{{{HD110315_N0_fit}}}
\includegraphics[scale=0.6]{{{HD110537_N0_fit}}}
\includegraphics[scale=0.6]{{{HD111031_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD11112_N0_fit}}}
\includegraphics[scale=0.6]{{{HD113490_N0_fit}}}
\includegraphics[scale=0.6]{{{HD115902_N0_fit}}}
\includegraphics[scale=0.6]{{{HD116258_N0_fit}}}
\includegraphics[scale=0.6]{{{HD118475_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD119782_N0_fit}}}
\includegraphics[scale=0.6]{{{HD120362_N0_fit}}}
\includegraphics[scale=0.6]{{{HD120780_N0_fit}}}
\includegraphics[scale=0.6]{{{HD123812_N0_fit}}}
\includegraphics[scale=0.6]{{{HD124523_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD125271_N0_fit}}}
\includegraphics[scale=0.6]{{{HD126203_N0_fit}}}
\includegraphics[scale=0.6]{{{HD126535_N0_fit}}}
\includegraphics[scale=0.6]{{{HD126614_N0_fit}}}
\includegraphics[scale=0.6]{{{HD127506_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD129445_N0_fit}}}
\includegraphics[scale=0.6]{{{HD131509_N0_fit}}}
\includegraphics[scale=0.6]{{{HD131664_N0_fit}}}
\includegraphics[scale=0.6]{{{HD13724_N0_fit}}}
\includegraphics[scale=0.6]{{{HD139189_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD144899_N0_fit}}}
\includegraphics[scale=0.6]{{{HD145675_N0_fit}}}
\includegraphics[scale=0.6]{{{HD147386_N0_fit}}}
\includegraphics[scale=0.6]{{{HD149782_N0_fit}}}
\includegraphics[scale=0.6]{{{HD149806_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD1502_N0_fit}}}
\includegraphics[scale=0.6]{{{HD150554_N0_fit}}}
\includegraphics[scale=0.6]{{{HD152079_N0_fit}}}
\includegraphics[scale=0.6]{{{HD15318_N0_fit}}}
\includegraphics[scale=0.6]{{{HD154682_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD155918_N0_fit}}}
\includegraphics[scale=0.6]{{{HD156146_N0_fit}}}
\includegraphics[scale=0.6]{{{HD156826_N0_fit}}}
\includegraphics[scale=0.6]{{{HD159062_N0_fit}}}
\includegraphics[scale=0.6]{{{HD164330_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD166599_N0_fit}}}
\includegraphics[scale=0.6]{{{HD167665_N0_fit}}}
\includegraphics[scale=0.6]{{{HD168769_N0_fit}}}
\includegraphics[scale=0.6]{{{HD16905_N0_fit}}}
\includegraphics[scale=0.6]{{{HD169889_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD17230_N0_fit}}}
\includegraphics[scale=0.6]{{{HD17354_N0_fit}}}
\includegraphics[scale=0.6]{{{HD175167_N0_fit}}}
\includegraphics[scale=0.6]{{{HD176110_N0_fit}}}
\includegraphics[scale=0.6]{{{HD176535_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD178340_N0_fit}}}
\includegraphics[scale=0.6]{{{HD181234_N0_fit}}}
\includegraphics[scale=0.6]{{{HD18143_N0_fit}}}
\includegraphics[scale=0.6]{{{HD183162_N0_fit}}}
\includegraphics[scale=0.6]{{{HD186408_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD188641_N0_fit}}}
\includegraphics[scale=0.6]{{{HD190067_N0_fit}}}
\includegraphics[scale=0.6]{{{HD195200_N0_fit}}}
\includegraphics[scale=0.6]{{{HD196385_N0_fit}}}
\includegraphics[scale=0.6]{{{HD199509_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD200083_N0_fit}}}
\includegraphics[scale=0.6]{{{HD201924_N0_fit}}}
\includegraphics[scale=0.6]{{{HD202206_N0_fit}}}
\includegraphics[scale=0.6]{{{HD203387_N0_fit}}}
\includegraphics[scale=0.6]{{{HD203473_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD203771_N0_fit}}}
\includegraphics[scale=0.6]{{{HD2039_N0_fit}}}
\includegraphics[scale=0.6]{{{HD203985_N0_fit}}}
\includegraphics[scale=0.6]{{{HD206025_N0_fit}}}
\includegraphics[scale=0.6]{{{HD206025_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD210797_N0_fit}}}
\includegraphics[scale=0.6]{{{HD213472_N0_fit}}}
\includegraphics[scale=0.6]{{{HD213519_N0_fit}}}
\includegraphics[scale=0.6]{{{HD214823_N0_fit}}}
\includegraphics[scale=0.6]{{{HD215257_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD217958_N0_fit}}}
\includegraphics[scale=0.6]{{{HD219077_N0_fit}}}
\includegraphics[scale=0.6]{{{HD219553_N0_fit}}}
\includegraphics[scale=0.6]{{{HD221146_N0_fit}}}
\includegraphics[scale=0.6]{{{HD223301_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD23439_N0_fit}}}
\includegraphics[scale=0.6]{{{HD24496_N0_fit}}}
\includegraphics[scale=0.6]{{{HD25311_N0_fit}}}
\includegraphics[scale=0.6]{{{HD25587_N0_fit}}}
\includegraphics[scale=0.6]{{{HD25912_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD26161_N0_fit}}}
\includegraphics[scale=0.6]{{{HD2638_N0_fit}}}
\includegraphics[scale=0.6]{{{HD26911_N0_fit}}}
\includegraphics[scale=0.6]{{{HD28185_N0_fit}}}
\includegraphics[scale=0.6]{{{HD37226_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD38230_N0_fit}}}
\includegraphics[scale=0.6]{{{HD38277_N0_fit}}}
\includegraphics[scale=0.6]{{{HD40397_N0_fit}}}
\includegraphics[scale=0.6]{{{HD4113_N0_fit}}}
\includegraphics[scale=0.6]{{{HD457_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD4614_N0_fit}}}
\includegraphics[scale=0.6]{{{HD56380_N0_fit}}}
\includegraphics[scale=0.6]{{{HD56957_N0_fit}}}
\includegraphics[scale=0.6]{{{HD60574_N0_fit}}}
\includegraphics[scale=0.6]{{{HD61383_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD62364_N0_fit}}}
\includegraphics[scale=0.6]{{{HD62549_N0_fit}}}
\includegraphics[scale=0.6]{{{HD6558_N0_fit}}}
\includegraphics[scale=0.6]{{{HD70642_N0_fit}}}
\includegraphics[scale=0.6]{{{HD71881_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD72440_N0_fit}}}
\includegraphics[scale=0.6]{{{HD72659_N0_fit}}}
\includegraphics[scale=0.6]{{{HD72892_N0_fit}}}
\includegraphics[scale=0.6]{{{HD74014_N0_fit}}}
\includegraphics[scale=0.6]{{{HD75881_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD80275_N0_fit}}}
\includegraphics[scale=0.6]{{{HD80883_N0_fit}}}
\includegraphics[scale=0.6]{{{HD80913_N0_fit}}}
\includegraphics[scale=0.6]{{{HD85440_N0_fit}}}
\includegraphics[scale=0.6]{{{HD85472_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD86006_N0_fit}}}
\includegraphics[scale=0.6]{{{HD8648_N0_fit}}}
\includegraphics[scale=0.6]{{{HD86950_N0_fit}}}
\includegraphics[scale=0.6]{{{HD89391_N0_fit}}}
\includegraphics[scale=0.6]{{{HD90520_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HD93489_N0_fit}}}
\includegraphics[scale=0.6]{{{HD97037_N0_fit}}}
\includegraphics[scale=0.6]{{{HD9796_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP101846_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP103019_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HIP110156_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP111854_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP111958_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP112918_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP116838_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HIP117219_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP1276_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP14729_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP19976_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP22059_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HIP22203_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP35965_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP41130_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP45839_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP46199_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HIP48953_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP52296_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP52942A_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP55507_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP55915_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HIP56489_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP59496_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP60910_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP61495_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP63762_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}
\begin{figure}
\includegraphics[scale=0.6]{{{HIP65956_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP78395_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP78408_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP948_N0_fit}}}
\includegraphics[scale=0.6]{{{HIP94931_N0_fit}}}
\caption{Similar to Fig. \ref{fig:fit1} but for other targets.}
\end{figure}

